Bayes-optimal Learning of Deep Random Networks of Extensive-width

We consider the problem of learning a target function corresponding to a deep, extensive-width, non-linear neural network with random Gaussian weights. We consider the asymptotic limit where the number of samples, the input dimension and the network width are proportionally large. We propose a closed-form expression for the Bayes-optimal test error, for regression and classification tasks. We further compute closed-form expressions for the test errors of ridge regression, kernel and random features regression. We find, in particular, that optimally regularized ridge regression, as well as kernel regression, achieve Bayes-optimal performances, while the logistic loss yields a near-optimal test error for classification. We further show numerically that when the number of samples grows faster than the dimension, ridge and kernel methods become suboptimal, while neural networks achieve test error close to zero from quadratically many samples.

==> trash.tex <==
The computation of the bracketed average can be carried out using the replica trick, observing
\begin{align}
    \left\langle\mathrm{sign}\left(\frac{1}{\sqrt{k_L}}a^\top h_L(x)\right)\right\rangle&=\mathbb{E}_{\mathcal{D},a_\star,\{W^\star_\ell\}_\ell}\underset{s\rightarrow 0}{\lim} Z^{s-1}\int da P_a(a)\prod\limits_{\ell}^LdW_\ell P_w(W_\ell) \prod\limits_{\mu=1}^nP_{\mathrm{out}}(y^\mu|\hat{y}(x^\mu))\mathrm{sign}\left(\hat{y}(x)\right)\notag\\
    &=\mathbb{E}_{\mathcal{D},a_\star,\{W^\star_\ell\}_\ell}\int \prod\limits_{a=1}^sda^a P_a(a^a)\prod\limits_{a=1}^s\prod\limits_{\ell}^LdW_\ell^a P_w(W_\ell^a) \prod\limits_{\mu=1}^n\prod\limits_{a=1}^sP_{\mathrm{out}}(y^\mu|\hat{y}^a(x^\mu)) \mathrm{sign}\left(\hat{y}^1(x)\right)
\end{align}
where $\hat{y}^1$ is the first replica of the student \eqref{eq:student}, with weights $a^a, \{W^a_\ell\}$. It follows that
\begin{align}
    \left\langle\mathrm{sign}\left(\frac{1}{\sqrt{k_L}}a^\top h_L(x)\right)\right\rangle ^k 
    &=\mathbb{E}_{\mathcal{D},a_\star,\{W^\star_\ell\}_\ell}\int \prod\limits_{a=1}^s\prod\limits_{\alpha=1}^k da^{a\alpha}P_a(a^{a\alpha})\prod\limits_{a=1}^s 
\prod\limits_{\alpha=1}^k\prod\limits_{\ell}^LdW_\ell^{a\alpha} P_w(W_\ell^{a\alpha})\notag\\ &~~~~\prod\limits_{\mu=1}^n\prod\limits_{\alpha=1}^k \mathrm{sign}\left(\hat{y}^{1\alpha}(x)\right)\prod\limits_{a=1}^sP_{\mathrm{out}}(y^\mu|\hat{y}^{a\alpha}(x^\mu)) ,
\end{align}
with the power $k$ effectively introducing a second level of replication. 
\begin{align}
    \mathbb{E}_{x}\mathbb{E}_{
    a_\star,\{W^\star_\ell\}_\ell}
    &\Theta\left[
   \frac{1}{\sqrt{k_L}}a_\star^\top h_L^\star(x)\times v
    \right]\left\langle\mathrm{sign}\left(\frac{1}{\sqrt{k_L}}a^\top h_L(x)\right)\right\rangle^k\notag\\ &
    =\mathbb{E}_{\mathcal{D},a_\star,\{W^\star_\ell\}_\ell}\int \prod\limits_{a=1}^s\prod\limits_{\alpha=1}^k da^{a\alpha}P_a(a^{a\alpha})\prod\limits_{a=1}^s 
\prod\limits_{\alpha=1}^k\prod\limits_{\ell}^LdW_\ell^{a\alpha} P_w(W_\ell^{a\alpha})\notag\\ &~~~~~~\mathbb{E}_{\{x^\mu\}_{\mu=1}^n}\prod\limits_{\mu=1}^n  \prod\limits_{a=1}^s\prod\limits_{\alpha=1}^kP_{\mathrm{out}}(y^\mu|\hat{y}^{a\alpha}(x^\mu)) \mathbb{E}_x \prod\limits_{\alpha=1}^k \mathrm{sign}\left(\hat{y}^{1\alpha}(x)\right)\Theta(v\times y(x) )\notag\\
&=e^{-skd f} \underbrace{\int \frac{1}{\sqrt{\det[2\pi Q]}} dh^0 \prod\limits_{0\le \alpha,\beta\le k} dh^\alpha e^{-\frac{1}{2}\sum\limits_{\alpha,\beta}h^\alpha h^\beta (Q^{-a})_{\alpha\beta}}\mathrm{sign}(h^\alpha)\Theta(v\times h^0)}_*
\end{align}
with $f$ the multilayer free energy of Appendix \ref{App:multilayer}. We used thefact that, since the underbraced term is not extensive, the rest of the integral concentrates around the same overlaps as discussed in Appendix \ref{App:multilayer}, leading to the $\exp{sdk \times f}$ factor. We denote, assuming replica symmetry, for $\alpha,\beta \ne 0$
\begin{equation}
Q_{\alpha\beta}:=\delta_{\alpha\beta}(\overline{r}-\overline{q})+\overline{q}:=\delta_{\alpha,\beta}\left[\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2(r^L_1-q^L_1)+\sum\limits_{\ell_0=1}^{L-1}\kappa_*^{(\ell_0)}\prod\limits_{\ell=\ell_0+1}^L\left(\kappa_1^{(\ell)}\right)^2r^L_{\ell_0+1}+\left(\kappa_*^{L}\right)^2r_a\right]+\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2q^L_1.
\end{equation}
and
\begin{align}
    &Q_{\alpha 0}:=\overline{m}:=\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2m^L_1\notag\\
&Q_{00}:=\overline{\rho}:=\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2\rho^L_1+\sum\limits_{\ell_0=1}^{L-1}\kappa_*^{(\ell_0)}\prod\limits_{\ell=\ell_0+1}^L\left(\kappa_1^{(\ell)}\right)^2\rho^L_{\ell_0+1}+\left(\kappa_*^{L}\right)^2\rho_a,
\end{align}
where we employ the notations of Appendix \ref{App:multilayer}. Note that in the Bayes optimal case, $\overline{r}=\overline{\rho}$ and $\overline{m}=\overline{q}$ due to the Nishimori identities, see Appendix \ref{App:multilayer}. The inverse $Q^{-1}$ has the same hierarchical structure as $Q$, with corresponding elements $\Tilde{\rho},\Tilde{m},\Tilde{r},\Tilde{q}$, which can be computed as \cite{Cui2019LargeDF}
\begin{align}
    \begin{cases}
        \Tilde{\rho}=\frac{\overline{r}+(k-1)\overline{q}}{\overline{\rho}(\overline{r}+(k-1)\overline{q})-k\overline{m}^2}\\
        \Tilde{r}=\frac{\overline{\rho}(\overline{r}+(k-2)\overline{q})-(k-1)\overline{m}^2}{(\overline{r}-\overline{q})(\overline{\rho}(\overline{r}+(k-1)\overline{q})-k\overline{m}^2)}\\
        \Tilde{m}=\frac{-m}{\overline{\rho}(\overline{r}+(k-1)\overline{q})-k\overline{m}^2}\\
        \Tilde{q}=\frac{\overline{m}^2-\overline{\rho}\overline{q}}{(\overline{r}-\overline{q})(\overline{\rho}(\overline{r}+(k-1)\overline{q})-k\overline{m}^2)}
    \end{cases}
\end{align}
{\color{red} WRONG!! Seem to have taken the $k=0$ limit here. Wrong, to fix!!}
. The curious reader is referred to \cite{Cui2019LargeDF} for a full detailed derivation in a related case. The end result is
\begin{align}
    *=\mathbb{E}_{\eta,h\sim\mathcal{N}(0,1)}\left[
\mathrm{erf}\left(
\sqrt{\frac{\overline{m}^2-\overline{\rho}\overline{q}}{\overline{\rho}(\overline{q}-\overline{r})}}\eta+\sqrt{\frac{\overline{m}^2}{\overline{\rho}(\overline{r}-\overline{q})}}h
\right)
    \right]^k \Theta[h\times v].
\end{align}
Plugging back in the expression of $\epsilon_g$:
\begin{align}
    1-\epsilon_g&=\int \dd v \dd \hat{v}e^{-iv\hat{v}}\sum\limits_{k=0}^\infty 
    \frac{(i\hat{v})^k}{k!}\mathbb{E}_{\eta,h\sim\mathcal{N}(0,1)}\left[
\mathrm{erf}\left(
\sqrt{\frac{\overline{m}^2-\overline{\rho}\overline{q}}{\overline{\rho}(\overline{q}-\overline{r})}}\eta+\sqrt{\frac{\overline{m}^2}{\overline{\rho}(\overline{r}-\overline{q})}}h
\right)
    \right]^k \Theta[h^0\times v]\notag\\
&=\mathbb{E}_{\eta,h\sim\mathcal{N}(0,1)} \Theta\left[
h\times \mathrm{erf}\left(
\sqrt{\frac{\overline{m}^2-\overline{\rho}\overline{q}}{\overline{\rho}(\overline{q}-\overline{r})}}\eta+\sqrt{\frac{\overline{m}^2}{\overline{\rho}(\overline{r}-\overline{q})}}h
\right)
\right]\notag\\
&=\mathbb{E}_{\eta,h\sim\mathcal{N}(0,1)} \Theta\left[
h\times \left(
\sqrt{\frac{\overline{\rho}\overline{q}}{\overline{m}^2}-1}\eta+h
\right)
\right]\notag\\
&=1-\frac{1}{\pi}\arccos\left[\sqrt{\frac{\overline{m}^2}{\overline{\rho}\overline{q}}}\right]\notag\\
&=1-\frac{1}{\pi}\arccos\left[\sqrt{\frac{\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2q^L_1}{\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2\rho^L_1+\sum\limits_{\ell_0=1}^{L-1}\kappa_*^{(\ell_0)}\prod\limits_{\ell=\ell_0+1}^L\left(\kappa_1^{(\ell)}\right)^2\rho^L_{\ell_0+1}+\left(\kappa_*^{L}\right)^2\rho_a}}\right]\notag\\
&=1-\frac{1}{\pi}\arccos\left(\frac{ \sqrt{\prod\limits_{\ell=1}^L\left(\kappa_1^{(\ell)}\right)^2q}}{{\sqrt{\Delta_a\int 
 z\dd \mu(z)\prod\limits_{\ell=1}^L \left(\kappa_1^{(\ell)}\right)^2\Delta_\ell+\epsilon_r}}} \right),
\end{align}
which concludes the derivation of \eqref{eq:error_classif}.
